DeliGrasp: Inferring Object Properties with LLMs for Adaptive Grasp Policies

Large language models (LLMs) can provide rich physical descriptions of most worldly objects, allowing robots to achieve more informed and capable grasping. We leverage LLMs' common sense physical reasoning and code-writing abilities to infer an object's physical characteristics$\unicode{x2013}$mass $m$, friction coefficient $\mu$, and spring constant $k$$\unicode{x2013}$from a semantic description, and then translate those characteristics into an executable adaptive grasp policy. Using a two-finger gripper with a built-in depth camera that can control its torque by limiting motor current, we demonstrate that LLM-parameterized but first-principles grasp policies outperform both traditional adaptive grasp policies and direct LLM-as-code policies on a custom benchmark of 12 delicate and deformable items including food, produce, toys, and other everyday items, spanning two orders of magnitude in mass and required pick-up force. We then improve property estimation and grasp performance on variable size objects with model finetuning on property-based comparisons and eliciting such comparisons via chain-of-thought prompting. We also demonstrate how compliance feedback from DeliGrasp policies can aid in downstream tasks such as measuring produce ripeness. Our code and videos are available at: https://deligrasp.github.io

==> tex/scrap.tex <==
% \vspace{-14pt}
\begin{figure}[!th]
    \centering
    % \includegraphics[width=0.70\columnwidth]{img/fbd_v4.png}
    % \includegraphics[width=0.70\linewidth]{img/fbd_v3.5.png}
    \includegraphics[width=1.0\linewidth]{img/setup_fbd_delidata.png}
    % \vspace{-12pt}
    \captionof{figure}{\textbf{A.} Our experimental setup with a tabletop UR5 robot arm equipped with the MAGPIE Gripper \citep{magpie} \textbf{B.} Free body diagram describing gripper interactions with an object at rest, adapted from \citep{adaptive_grasp} \textbf{C.} The delicate objects dataset.}
    \label{fig:fbd}
   \vspace{-12pt}
\end{figure}

\begin{table}[!th]
\scriptsize
\centering
\captionof{table}{\scriptsize{DeliGrasp Model Comparisons of Estimated $F_{min}$ and \textit{m} }}
\label{tab:dg_VS_dg_direct}
\begin{tabular}{@{}lllll|llllll|ll|llll|llll|llll}
\toprule
&  Ground Truth& &&&   $DG$ &&&   & & & $DG$&$D$ & $DG$&$FT$ &   && $DG$&$CoT$ &&& $DG$&$FT$& $CoT$ &\\
 ID &  Object Name &  $F$&$m$ &$k$ &   $F$&$F$&$m$ & $m$ & $\mu$&$k$ & $F$&$F$& $F$&$F$&   $m$&$m$ & $F$&$F$&$m$& $m$ & $F$&$F$& $m$&$m$ \\
   &    & (N)        
&(g) &(N/m)&   (N)        
&
\textit{Err.} &(g) &  \textit{Err.}& &(N/m)             
 & (N)        
&\textit{Err.}  & (N)        
&\textit{Err.} &   (g)&\textit{Err.}  & (N)        
&\textit{Err.} &(g)&\textit{Err.} & (N)        
&\textit{Err.} & (g)&\textit{Err.} \\
\midrule
1  &  Paper Airplane &  0.02&0.8&184.9&   0.10&\textit{0.08}
&5
 &  \textit{6.25}
 & 0.5 &20   
 & 0.15 
&\textit{0.13} 
 & 0.10
&\textit{ 0.08  }
&   5
&\textit{6.25}
 &  0.10
&\textit{ 0.08  }
&5
&\textit{6.25}
 &  0.02
&\textit{ 0.00  }
& 1
&\textit{1.25}
 \\
2  &  Cup (empty) &  0.11
&3.6&389.8&   0.25  &\textit{0.14}
&10
 &  \textit{2.78}
 & 0.4 &50   
 & 0.5  
&\textit{0.39} 
 & 0.25
&\textit{ 0.14  }
&   10
&\textit{2.78}
 & 0.12
&\textit{ 0.01  }
&5
&\textit{1.39}
 & 0.12
&\textit{ 0.01  }
& 5
&\textit{1.39}
 \\
3  &  Dried Yuba  &  0.16
&5.5&157.7&   0.39  &\textit{0.23}
&20
 &  \textit{3.64}
 & 0.5 &200  
 & 0.5  
&\textit{0.34} 
 & 0.39
&\textit{ 0.23  }
&   20
&\textit{3.64}
 & 0.20
&\textit{ 0.04  }
&10
&\textit{1.82}
 & 0.20
&\textit{ 0.04  }
& 10
&\textit{1.82}
 \\
4  &  Raspberry &  0.18
&6&61.0&   0.06&\textit{0.12}
&5
 &  \textit{1.17}
 & 0.8 &50   
 & 0.2  
&\textit{0.02} 
 & 0.25
&\textit{ 0.07  }
&   20
&\textit{3.33}
 & 0.05
&\textit{ 0.13  }
&4
&\textit{1.33}
 & 0.06
&\textit{ 0.12  }
& 5
&\textit{1.17}
 \\
5  &  Hard Taco  &  0.44
&15&188.4&   0.98  &\textit{0.54}
&50
 &  \textit{3.33}
 & 0.5 &1000 
 & 1.5  
&\textit{1.06} 
 & 0.20
&\textit{ 0.24  }
&   10
&\textit{1.33}
 & 0.59
&\textit{ 0.15  }
&30
&\textit{2.00}
 & 0.20
&\textit{ 0.24  }
& 10
&\textit{1.33}
 \\
6  &  Mandarin &  1.65
&56&151.8&   1.88  &\textit{0.23}
&150
 &  \textit{2.68}
 & 0.8 &500  
 & 1.25 
&\textit{0.40} 
 & 1.84
&\textit{ 0.19  }
&   150
&\textit{2.68}
 & 0.92
&\textit{ 0.73  }
&75
&\textit{1.34}
 & 0.61
&\textit{ 1.04  }
& 50
&\textit{1.11}
 \\
7  &  Stuffed Toy &  2.18
&74&192.8&   0.61  &\textit{1.57}
&50
 &  \textit{1.32}
 & 0.8 &100  
 & 1.5  
&\textit{0.68} 
 & 0.61
&\textit{ 1.57  }
&   50
&\textit{1.32}
 & 0.37
&\textit{ 1.81  }
&30
&\textit{1.59}
 & 0.25
&\textit{ 1.93  }
& 20
&\textit{1.73}
 \\
8  &  Cup (water)  &  3.12
&106&373.2&   4.08  &\textit{0.96}
&250
 &  \textit{2.36}
 & 0.6 &200  
 & 3&   
\textit{0.12} & 3.27
&\textit{ 0.15  }
&   200
&\textit{1.89}
 & 1.64
&\textit{ 1.49  }
&100
&\textit{1.06}
 & 2.45
&\textit{ 0.67  }
& 150
&\textit{1.42}
 \\  
9  &  Bag (noodles) &  5.62
&191&4324.&   12.3  &\textit{6.68}
&500
 &  \textit{2.62}
 & 0.4 &300  
 & 4&   
\textit{1.62} & 4.91
&\textit{ 0.72  }
&   200
&\textit{1.05}
 & 6.13
&\textit{ 0.51  }
&250
&\textit{1.31}
 & 4.91
&\textit{ 0.72  }
& 200
&\textit{1.05}
 \\   
10 &  Avocado  &  6.00
&204&298.7&   3.92  &\textit{2.08 }
&200
 &  \textit{1.02}
 & 0.5 &500  
 & 1&   
\textit{5.00} & 3.92
&\textit{ 2.08  }
&   200
&\textit{1.02}
 & 2.94
&\textit{ 3.06  }
&150&\textit{1.26}
 & 3.92
&\textit{ 2.08  }
& 200&\textit{1.02}
 \\  
11 &  Spray Bottle  &  7.36
&250&1383.&   12.2  &\textit{4.84 }
&500
 &  \textit{2.00}
 & 0.4 &150  
 & 5&   
\textit{2.36} & 7.36
&\textit{ 0.00  }
&   300
&\textit{1.20}
 & 8.58
&\textit{ 1.22  }
&350
&\textit{1.40}
 & 11.0
&\textit{ 3.68  }
& 450
&\textit{1.80}
 \\   
12 &  Bag (rice) &  26.5&900&6192.&   19.6  &\textit{5.9  }&1000 &  \textit{1.11} & 0.5 &200   & 8&   \textit{18.5} & 19.6&\textit{ 6.87 } &   1000&\textit{1.11} & 19.6&\textit{ 6.87 } &1000&\textit{1.11} & 19.6&\textit{ 6.87 } & 1000&\textit{1.11} \\   
\bottomrule
\end{tabular}
\caption*{We record LLM estimates for $F$, the minimum grasping force, the absolute error $F$ $Err.$, mass $m$, and ratio of mass overestimation $m$ $Err.$ for 5 different DeliGrasp strategies: $DG$ with the default model without finetuning, the ablated $DG D$ which directly estimates $F$, $DG$ $FT$ with the model finetuned on the PhysObjects dataset, $DG$ $CoT$ for the non-finetuned model with additional chain-of-thought prompting, and $DG$ $FT$ $CoT$ for the finetuned model with additional chain-of-thought prompting. We use the same $\mu$ and $k$ values across models to isolate the effect of mass estimates on grasping. }
\end{table}

\begin{table}[ht]
\centering
\begin{minipage}[b]{0.65\linewidth}
\scriptsize
\centering
\captionof{table}{\scriptsize{DeliGrasp Model Comparisons of Estimated $F_{min}$ and \textit{m} }}
\label{tab:dg_VS_dg_direct}
\begin{tabular}{@{}lcccc@{}llllllll}
\toprule
ID & $F_{DG}$ & $F_{DG}$ & $F_{DG}$& $F_{DG}$& $m_{DG}$&  $m_{DG}$&   $m_{DG}$&$m_{DG}$&$m_{DG}$&$m_{DG}$
& $m_{FT}$&$m_{FT}$\\
 & & & $_{-D}$& $_{-D}$& & &   $_{-FT}$&$_{-FT}$&$_{-CoT}$& $_{-CoT}$& $_{-CoT}$&$_{-CoT}$\\
   &  (N)     & \textit{Err.} (N) & (N)        & \textit{Err.} (N)        & (g)&  \textit{Err.} (g)&   (g)&\textit{Err.} (g)&(g)&\textit{Err.} (g)& (g)&\textit{Err.} (g)\\
\midrule
1  & 0.10  & \textit{0.08}& 0.15 & \textit{0.13} & 5
&  \textit{6.25}
&   5
&\textit{6.25}
&5
&\textit{6.25}
& 1
&\textit{1.25}
\\
2  & 0.25  & \textit{0.14 }& 0.5  & \textit{0.39} & 10
&  \textit{2.78}
&   10
&\textit{2.78}
&5
&\textit{1.39}
& 5
&\textit{1.39}
\\
3  & 0.39  & \textit{0.23 }& 0.5  & \textit{0.34} & 20
&  \textit{3.64}
&   20
&\textit{3.64}
&10
&\textit{1.82}
& 10
&\textit{1.82}
\\
4  & 0.06  & \textit{0.12 }& 0.2  & \textit{0.02} & 5
&  \textit{1.17}
&   20
&\textit{3.33}
&4
&\textit{1.33}
& 5
&\textit{1.17}
\\
5  & 0.98  & \textit{0.54 }& 1.5  & \textit{1.06} & 50
&  \textit{3.33}
&   10
&\textit{1.33}
&30
&\textit{2.00}
& 10
&\textit{1.33}
\\
6  & 1.88  & \textit{0.23 }& 1.25 & \textit{0.40} & 150
&  \textit{2.68}
&   150
&\textit{2.68}
&75
&\textit{1.34}
& 50
&\textit{1.11}
\\
7  & 0.61  & \textit{1.57 }& 1.5  & \textit{0.68} & 50
&  \textit{1.32}
&   50
&\textit{1.32}
&30
&\textit{1.59}
& 20
&\textit{1.73}
\\
8  & 4.08  & \textit{0.96}& 3	   & \textit{0.12} & 250
&  \textit{2.36}
&   200
&\textit{1.89}
&100
&\textit{1.06}
& 150
&\textit{1.42}
\\  
9  & 12.3  & \textit{6.68}& 4	   & \textit{1.62} & 500
&  \textit{2.62}
&   200
&\textit{1.05}
&250
&\textit{1.31}
& 200
&\textit{1.05}
\\   
10 & 3.92  & \textit{2.08}& 1	   & \textit{5.00} & 200
&  \textit{1.02}
&   200
&\textit{1.02}
&150&\textit{1.26}
& 200&\textit{1.02}
\\  
11 & 12.2  & \textit{4.84}& 5	   & \textit{2.36} & 500
&  \textit{2.00}
&   300
&\textit{1.20}
&350
&\textit{1.40}
& 450
&\textit{1.80}
\\   
12 & 19.6  & \textit{5.9}& 8	   & \textit{18.5} & 1000&  \textit{1.11}&   1000&\textit{1.11}&1000&\textit{1.11}& 1000&\textit{1.11}\\   
\bottomrule
\end{tabular}
\end{minipage}
\hfill
\begin{minipage}[b]{0.3\linewidth}
\scriptsize
\centering
\captionof{table}{\scriptsize{Model comparison of mass estimates and grasping success for a typical (143g) and large (306g) avocado}}
\label{tab:model_comparison}
\begin{tabular}{@{}lccccc@{}}
\hline
\textbf{Model} & \textbf{DG} & \textbf{DG} & \textbf{DG} & \textbf{DG} \\
&   & \textbf{FT} & \textbf{CoT} & \textbf{FT CoT} \\
\hline
$A_1$ $1^{st}$ Query \\
\hline
\textit{m} (g) & 200 & 200 & 150 & 200 \\
Success& 100\% & 100\% & 100\% & 100\%  \\
\hline
$A_2$ $1^{st}$ Query \\
\hline
\textit{m} (g) & 200 & 200 & 250 & 300  \\
Success & 20\% & 10\% & 80\% & 100\%  \\
\hline
$A_2$ $2^{nd}$ Query \\
\hline
\textit{m} (g) & 300 & 300 & 400 & --- \\
Success & 100\% & 100\% & 100\% & ---  \\
\bottomrule
\end{tabular}
\end{minipage}
\hfill
\end{table}

\subsubsection{LLM Force and \textit{k} Prediction Accuracy}
Three column table replicating rows from above delicate object table. First column shows LLM estimated minimal grasping force. Second column shows "ground truth" estimated grasp force w/ 20\% safety margin. Third column shows squared error. 
\begin{table}[h]
    \centering
    \vspace{-6pt}
    \caption{LLM Force and Spring Constant Prediction Correctness}
    \label{tab:multistep_ripeness}
    \begin{tabular}{lccccc}
        \toprule
         Object & $F_{a_{LLM}}$ & $F_a$ MSE & $k_{LLM}$ & $k$ SE\\
          & (N) & (N) & (N/m) & (N/m)\\
        \midrule
        Paper Airplane    & 0.98 & 0.748  & &  \\
        Cup (empty)       & 0.92 & 0.699  & &  \\
        Dried Yuba        & 1.14 & 1.183  & &  \\
        Raspberry         & 0.83 & 0.418  & &  \\
        Hard Taco         & 6.70 & 40.68  & &  \\
        Mandarin          & 2.01 & 0.222  & &  \\
        Stuffed Toy       & 1.60 & 0.104  & &  \\
        Cup (water)       & 2.88 & 0.613  & &  \\
        Bag (noodles)     & 12.0 & 39.74  & &  \\
        Ripe Avocado      & 4.20 & 4.862  & &  \\
        Spray Bottle      & 16.1 & 96.99  & &  \\
        Bag (rice)        & 1.50 & 625    & &  \\
    \bottomrule
    \end{tabular}
\end{table}

\subsection{YCB Benchmark}
To establish a floor of grasp skills, we compare L2G on the YCB benchmark against two other grasp strategies: a traditional uniform closing of the gripper and a closing of the gripper to a perception-determined object width. Full YCB benchmark test data can be seen in Appendix \ref{appendix:ycb}. 
